Bridging Modalities and Transferring Knowledge: Enhanced Multimodal Understanding and Recognition

This manuscript explores multimodal alignment, translation, fusion, and transference to enhance machine understanding of complex inputs. We organize the work into five chapters, each addressing unique challenges in multimodal machine learning. Chapter 3 introduces Spatial-Reasoning Bert for translating text-based spatial relations into 2D arrangements between clip-arts. This enables effective decoding of spatial language into visual representations, paving the way for automated scene generation aligned with human spatial understanding. Chapter 4 presents a method for translating medical texts into specific 3D locations within an anatomical atlas. We introduce a loss function leveraging spatial co-occurrences of medical terms to create interpretable mappings, significantly enhancing medical text navigability. Chapter 5 tackles translating structured text into canonical facts within knowledge graphs. We develop a benchmark for linking natural language to entities and predicates, addressing ambiguities in text extraction to provide clearer, actionable insights. Chapter 6 explores multimodal fusion methods for compositional action recognition. We propose a method fusing video frames and object detection representations, improving recognition robustness and accuracy. Chapter 7 investigates multimodal knowledge transference for egocentric action recognition. We demonstrate how multimodal knowledge distillation enables RGB-only models to mimic multimodal fusion-based capabilities, reducing computational requirements while maintaining performance. These contributions advance methodologies for spatial language understanding, medical text interpretation, knowledge graph enrichment, and action recognition, enhancing computational systems' ability to process complex, multimodal inputs across diverse applications.

==> chapters/abstract/abstract.tex <==
% !TeX root = ../../thesis.tex
\chapter{Abstract}\label{ch:abstract}
In this manuscript, we explore the challenges of multimodal alignment, translation, fusion, and transference, and aim to significantly enhance multimodal machine understanding and recognition capabilities. We organize the work into five chapters, where each chapter addresses a unique challenge within the broader field of multimodal machine learning. The motivation behind this research is to bridge the gap between various data modalities, enabling machines to process and interpret complex, multimodal inputs in a manner akin to human cognition. By doing so, we seek to push the boundaries of what can be achieved in terms of automated scene generation, medical text navigation, knowledge graph enrichment, and action recognition.

In \textbf{Chapter~\ref{ch:emnlp2020}}, we introduce a novel method---Spatial-Reasoning Bert---designed for translating text-based spatial relations into 2D spatial arrangements between clip-arts. With the method we propose, we enable effective decoding of spatial language into visual representations. This capability paves the way for automated scene generation that closely aligns with human spatial understanding, addressing a critical need for intuitive and accurate spatial reasoning in computational systems.

In \textbf{Chapter~\ref{ch:conll2020}}, we shift our focus to the medical domain and present a novel method for accurately translating medical texts into specific 3D locations within an anatomical human atlas. We introduce a novel loss function that leverages the spatial co-occurrences of medical terms to create an interpretable mapping of medical knowledge. The method we propose significantly enhances the interpretability and navigability of medical texts.

In \textbf{Chapter~\ref{ch:emnlp2023}}, we explore the challenge of translating structured text into canonical facts within large-scale knowledge graphs. We develop a benchmark dataset for linking structured natural language text to entities and predicates within knowledge graphs, and make a substantial contribution toward improving the utility of often ambiguous information extracted from texts. The methods we propose tackle the inherent ambiguities in text extraction, offering clearer and more actionable insights from textual data.

In \textbf{Chapter~\ref{ch:bmvc2021}}, we research various multimodal fusion methods to improve compositional action recognition. We propose a novel action recognition method, which performs multimodal fusion of video frames and object detection representations, and improves the robustness and accuracy of action recognition. Overall, the work we conduct highlights the importance of fusion techniques in enhancing model performance.

Finally, in \textbf{Chapter~\ref{ch:iccv2023}} we delve into multimodal knowledge transference for egocentric action recognition, alleviating the practical limitations of \textbf{Chapter~\ref{ch:bmvc2021}}. In particular, we showcase how multimodal knowledge distillation can enable a model trained only on RGB frames to mimic the capabilities of a multimodal fusion-based model. This approach offers a pragmatic solution to reduce computational requirements while maintaining high performance.

Overall, through this manuscript, we offer substantial methodological advancements and new insights into overcoming the challenges inherent in multimodal machine learning. Through a series of actionable approaches to spatial language understanding for abstract scene generation, medical text interpretation, knowledge graph enrichment, and action recognition, this work significantly enhances computational systems' ability to understand and recognize complex, multimodal inputs across a range of applications.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/abstractnl/abstractnl.tex <==
% !TeX root = ../../thesis.tex
\chapter{Beknopte samenvatting}
In dit manuscript onderzoeken we de uitdagingen van multi-modale uitlijning, -vertaling, -fusie en -overdracht en streven ernaar belangrijke vorderingen te maken om machines beter te maken in multi-modaal begrip en herkenning. We verdelen het werk in 5 hoofdstukken, waar elk hoofdstuk een uniek stuk aanpakt in het bredere veld van multi-modaal machinaal leren. De motivatie achter dit onderzoek is een brug te slaan tussen verschillende soorten data en zo machines de mogelijkheid te geven om complexe multi-modale data te verwerken en interpreteren in een manier die aansluit bij de menselijke rede. Door dit te doen proberen we de grens te verleggen van wat er bereikt kan worden in automatische  scene generatie, medische tekst navigatie, kennisgrafiek verrijking en actieherkenning.

In \textbf{Chapter~\ref{ch:emnlp2020}}, introduceren we een nieuwe methode---Spatial-Reasoning Bert---die ontwikkelt is voor het vertalen van tekstgebaseerde ruimtelijke relaties naar 2D ruimtelijke overeenkomsten tussen clip-arts. Met deze voorgestelde methode, beogen we het effectief decoderen van ruimtelijke taal in visuele voorstellingen. Deze mogelijkheid baant de weg naar automatische scene generatie, die dicht aanleunt tegen menselijk ruimtelijk begrip, een kritische link voor intuïtief en accuraat ruimtelijk redeneren in computersystemen.

In \textbf{Chapter~\ref{ch:conll2020}}, verschuiven we onze aandacht naar het medische domein en stellen we een nieuwe methode voor, voor het accuraat vertalen van medische teksten naar specifieke 3D locaties binnen een anatomische menselijke atlas.  We introduceren een nieuwe verlies functie, die gebruikt wordt om het ruimtelijk gelijktijdig voorkomen van medische termen, medisch interpreteerbaar in kaart brengen. Deze methode verbetert significant de duidelijkheid en navigatiemogelijkheden van medische teksten.

In \textbf{Chapter~\ref{ch:emnlp2023}}, onderzoeken we de uitdaging van het vertalen van gestructureerde tekst naar canonieke feiten binnen grootschalige kennisgrafieken. We ontwikkelen een benchmark dataset voor het koppelen van gestructureerde natuurlijke teksten aan entiteiten en eigenschappen binnen kennisgrafieken en leveren een aanzienlijke bijdrage tot het verbeteren van de bruikbaarheid van vaak ambigue informatie, die uit teksten werd geëxtraheerd. De methoden die we voorstellen pakken de inherente ambiguïteit aan in tekst extractie, waardoor er duidelijker en meer gebruiksklare inzichten ontstaan uit tekstuele data.

In \textbf{Chapter~\ref{ch:bmvc2021}}, onderzoeken we verschillende multi-modale fusie methoden ter verbetering van compositionele actieherkenning. We stellen een nieuwe actieherkenningsmethode voor, met de multi-modale fusie van videoframes en representaties van objectherkenning, die de robuustheid en accuraatheid van actieherkenning  verbetert. In het algemeen beklemtoont ons werk het belang van fusietechnieken in de verbetering van modellen.

Tenslotte, in \textbf{Chapter~\ref{ch:iccv2023}} duiken we in multi-modale kennisoverdracht voor egocentrische actieherkenning, waarbij we de praktische beperkingen verminderen van \textbf{Chapter~\ref{ch:bmvc2021}}. In het bijzonder laten we zien hoe het gebruik van multi-modale kennis, in een model getraind uitsluitend op basis van RGB frames,  de mogelijkheden kan nabootsen van een model gebaseerd op multi-modale fusie. Deze aanpak biedt een pragmatische oplossing  voor verlaagde eisen aan rekenkracht, zonder verlies aan performantie.

In zijn algemeenheid en tijdens dit hele manuscript, bieden we substantiële  methodologische vooruitgang en nieuwe inzichten, om de uitdagingen inherent aan multi-modaal machinaal leren aan te pakken. Door een serie van handelingen in het begrijpen van ruimtelijke taal voor abstracte scene generatie, medische tekst interpretatie, verrijking van kennisgrafieken en actieherkenning, helpt dit werk significant om computersystemen vooruit te helpen in het begrijpen en herkennen van complexe, multi-modale input voor een scala aan toepassingen.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/curriculum/curriculum.tex <==
% !TeX root = ../../thesis.tex
\chapter{Curriculum}\label{ch:curriculum}
Gorjan Radevski was born on 17.05.1994 in Skopje, Republic of North Macedonia. He received his Bachelor's Degree in Computer Science from the Ss. Cyril and Methodius University in Skopje (2017). He later obtained his Master's Degree at the Faculty of Engineering Science of KU Leuven -- Department of Computer Science (2019). During his master's studies he did machine learning (research) internships at Luminovo in Munich, Germany, and IBM Research in Zurich, Switzerland, where he worked with Dr. Jasmina Bogojeska. Later, in 2019, he joined the Visics Group of the Department of Electrical Engineering (ESAT), to pursue the PhD degree under the supervision of Prof. Tinne Tuytelaars and Prof. Marie-Francine Moens. Towards the end of his PhD, he did a research internship at NEC Labs in Heidelberg, Germany, where he worked with Dr. Kiril Gashteovski, Dr. Caroline Lawrence, and Prof. Goran Glavaš.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}

==> chapters/epilogue_part_i/epilogue_part_i.tex <==
\chapter*{Epilogue of Part I}\label{ch:epilogue_part_i}

We contribute towards addressing \inlineuniversalresearchquestion{Transversal Research Question I}.

\cleardoublepage

==> chapters/epilogue_part_ii/epilogue_part_ii.tex <==
\chapter*{Epilogue of Part II}\label{ch:epilogue_part_ii}
We contribute towards addressing \inlineuniversalresearchquestion{Transversal Research Question II}.

\cleardoublepage

==> chapters/manual/manual.tex <==
% !TeX root = ../../thesis.tex
\chapter{Manual}\label{ch:manual}


\section{Tips and Tricks}

\subsection{Image on the cover page}

If you want to place an image on the cover of the dissertation, you can add
the code underneath to the template (check with your promotor whether this is
allowed).

\paragraph{Include image:}
Search for the \texttt{\textbackslash frontcoverheaderXII} command in
the \texttt{adsphd.cls} file and add the following lines:
\begin{verbatim}
   \begin{textblock*}{56mm}(10mm+#1,15mm)
   \includegraphics[width=56mm,height=20mm]{image/filename}
   \end{textblock*}
\end{verbatim}
Where 56mm is the width, 20mm the height, 10mm the x-location and 15mm the
y-location.

\paragraph{Change cover font color:}
Add the command \texttt{\textbackslash color\{red\}} to the
\texttt{\textbackslash frontcoverheaderXII} command or enclose specific parts.
For example, \texttt{\{\textbackslash color\{red\}\textbackslash
textbf\{\textbackslash @authorf\textbackslash\ \textbackslash @authorl\}}.

\subsection{Full cover page}

\textbf{Important}: most printing services will create their own cover page based
on the details you send them (title, name, affiliation, ...) and do not supply
you with all necessary parameters (e.g., thickness of the paper) because these
differ from machine to machine. Therefore, the generated cover page is only
indicative and probably not used by your printing server (or even correct).


A full cover page (combining front cover, spine and back cover) can be
generated automatically using the command \texttt{make cover} or \texttt{python3 run.py cover}. This creates a pdf
\texttt{\$(COVERPDF);} by default this is \texttt{cover.pdf}.

The width of the spine is set by redefining \texttt{\\adsphdspinewidth} (9mm by default).

It can be seen in the provided \texttt{thesis.tex} that all information necessary to
generate a cover page is contained between two markers

\begin{verbatim}
    %%% COVER: Settings %%%
    ...
    %%% COVER: End settings %%%
\end{verbatim}

DO NOT REMOVE THESE!! They are used by the Makefile!!

The default front and/or back cover page can be overwritten: 

\begin{itemize}
    \item create a file \texttt{mycoverpage.tex}
    \item redefine the commands \texttt{\textbackslash makefrontcovergeneral} and \texttt{\textbackslash makebackcovergeneral}. For
          an example and more information, see the provided file \texttt{mycoverpage.tex}.
\end{itemize}

The cover page in the generated pdf has the following structure:

{\tiny
\begin{verbatim}
    <--rbleed--><--backcoverpage--><--lbleed--><--spine width--><--lbleed--><--frontcoverpage--><--rbleed-->
\end{verbatim}
}

The default bleed (both lbleed and rbleed) is 7mm. I suggest not changing this
value unless you know what you are doing ;) The latter can be done by
redefining \texttt{\textbackslash defaultlbleed} and \texttt{\textbackslash defaultrbleed} respectively.


\subsection{Table of contents}

To remove list of figures, tables and other preface chapters from the table of
contents, search for occurrences of \texttt{\textbackslash addcontentsline} in the file
\texttt{adsphd.cls} and comment them.

\subsection{Small ebook size}

When you add the \texttt{epub} option to the adsphd class the dissertation is
printed to a smaller size to read on a device such as Kindle.

Environments such as tables or tikZ pictures are often sized in absolute values
and not relative to the size of the output. You can wrap them in a resizebox
to enforce scaling:

\begin{verbatim}
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{cc}
      ...
    \end{tabular}
  }
\end{verbatim}

\section{Settings for TeXstudio}

If you are working with TeXstudio or other windows latex editors you might want to adjust the editor's settings to allow a proper compilation of the table of contents and list of figures/tables.

\subsection{Custom \textit{makeindex} and \textit{makeglossaries} commands}

According to the \textit{README.md} the tables are indexed through two custom commands. To edit them in TeXstudio open the \textit{Commands} settings (\textit{Options $\to$ Configure TeXstudio...,  Commands} sheet), edit the following fields and press OK.

\textit{Makeindex}:
{\scriptsize
\begin{verbatim}
"C:/Program Files/MiKTeX 2.9/miktex/bin/x64/makeindex.exe" %.nlo -s nomencl.ist -o %.nls
\end{verbatim}}

\textit{Makeglossaries}:
{\scriptsize
\begin{verbatim}
"C:/Program Files/MiKTeX 2.9/miktex/bin/x64/makeindex.exe" %.glo -s %.ist -t %.glg -o %.gls
\end{verbatim}}

Now the customized commands can be launched by using \textit{Tools $\to$ Commands $\to$ MakeIndex/Makeglossaries}. If you want to automatize it in the standard \textit{Build \& View} (F5) and \textit{Compile} (F6) commands look at the following section.

\subsection{Custom Build\&View and Compile meta-commands}

Open \textit{Options $\to$ Configure TeXstudio...,  Build} sheet, edit the following field and press OK.

\textit{Build \& View}:
{\footnotesize\begin{verbatim}
	txs:///pdflatex | txs:///bibtex | txs:///makeglossaries | txs:///makeindex |
	txs:///pdflatex  | txs:///pdflatex
	\end{verbatim}}

To view the PDF once created you have to press F7 (or \textit{Tool $\to$ View}) and the PDF will automatically update in the default viewer whan you modify it. 

If you prefer to directly view the created PDF\textbf{ from the beginning }edit the field as follow:
{\footnotesize\begin{verbatim}
	txs:///pdflatex | txs:///bibtex | txs:///makeglossaries | txs:///makeindex |
	txs:///pdflatex  | txs:///pdflatex | txs:///view-pdf
	\end{verbatim}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage



==> chapters/preamble_part_i/preamble_part_i.tex <==
\chapter*{Preamble of Part I}\label{ch:preamble_part_i}
\universalresearchquestion{Transversal Research Question I}{How effectively can we align and translate across different modalities to bridge the semantic gap between heterogeneous data forms, while accounting for the modality-specific nuances and challenges of out-of-distribution data?}
\cleardoublepage

==> chapters/preamble_part_ii/preamble_part_ii.tex <==
\chapter*{Preamble of Part II}\label{ch:preamble_part_ii}
\universalresearchquestion{Transversal Research Question II}{How can we harness the power of multimodal fusion and knowledge transference to create more capable and efficient video understanding machine learning models?}
\cleardoublepage

==> chapters/preface/preface.tex <==
% !TeX root = ../../thesis.tex
\chapter*{Acknowledgments}\label{ch:preface}

\epigraph{I find my solace in people.}{\textit{Dave Chapelle}}
Reflecting on the past five years, one term stands out: ``support''. Though it may seem I persevered alone, the unwavering support from those around me carried me through the many moments of uncertainty. I dedicate this to you.

To Tinne and Sien, my mentors\footnote{Prof. Tinne Tuytelaars and Prof. Marie-Francine Moens.}. Sien, I recall asking for your help when working on my first paper. Your comment: ``On Saturday I'll have to take care of my grandchildren, but on Sunday I'm free.'' Was the paper exceptional? Undoubtedly not. Tinne, I was feeling down at the end of 2021, and I impulsively booked a one-way flight home without discussing with you. When I informed you later that week, and apologized for not discussing with you first, you advised me that I go home and rest as much as I needed. The fact that both of you (most likely) don't remember these occurrences, says more than I could ever describe. I read a saying online\footnote{Some Reddit Ph.D.-related thread I think...} that we become a lot like our Ph.D. mentors; I sincerely hope I do. Thank you for your support, guidance, and understanding.

To all other members of the jury. Prof. Damen, it was wishful thinking for me to have you on the thesis committee. I hope it was worthwhile for you as well. Prof. Blockeel, before I applied for my Master's at KU Leuven, the first person I looked up online was my machine learning professor at the Master's programme. Today, I'm honored to have you on my Ph.D. committee. Prof. Van hamme, many of the below-mentioned know you as: ``The speech professor who, if you google, you'll see images of him doing triathlons''. I find that super inspiring! Prof. Willems, I'm humbled to have you as the chair. Prof. Glavaš, I mention you in the ``friends and family'' part. I thank you all!

To my PSI\footnote{Abbreviated from Processing Speach and Images, the group I'm part of.} (ex-)colleagues, especially the group I've spent most time with, in no particular order: Tim, Timm, Abhishek, Cedric, Eli, Thomas, Matthias, George, Fanis, Bo, Junyi; I'm glad to have (had) you as my colleagues! The same goes for everyone else, whom I forgot to mention by name here. To all other PSI staff. Paul Konijn---who allows us to do research by doing everything else for us---we would have had the defense outdoors without your help. Bert DeKnuydt (our system admin), my teaching assistant duties would have been impossible without your help. Patricia, Annitta, Kim, and Wim, among other things, you handle my contracts and reimburse my travel expenses---contributing to a positive bank account balance! Sincere thanks to you all.

I was also fortunate to meet a lot of wonderful people during my time in Belgium: both Leuven and Antwerp. To Draganica, although being your friend is sometimes costly: e.g., you somehow don't have your bank card often (?); during the Covid days, the only thing keeping me (half) sane were the evenings in the Campus Irena balcony. To Sandu (Dusan), it's not a surprise the best works I've done during the Ph.D. were with you. To Pejevce, when we arrived in Leuven, it was you who introduced us to everything. My Master's studies would have lasted way longer without your help. To Tea and Viktor. Tea, thank you for carrying me the past year, unfortunately, it's not easy...Viktor, I'm pretty sure the sofa at our place would still be half-assembled without your help. To Aiste, Pablo, and Keyvan, as you made Antwerp feel like home to us. Thank you all for the good times together, and the many more to come.

To the people I met during my time at NEC, Kirca and Bile. To Kirca, for being the most selfless person I know. Both of you are among the nicest people I have met, and I'm happy to call you friends. To Goran\footnote{Prof. Goran Glavaš, member of the Ph.D. jury, and supervisor during my NEC internship.}, perhaps the most sharp-witted and humble person I know.
Despite having a newborn and a packed schedule, you agreed to be on the thesis committee, came to Leuven for the preliminary defense, and spent the whole day (literally!) sharing your thoughts on everything with me. I'm truly grateful to have met all of you.

To the people I know longer than I don't, prefixed by ``Bate''\footnote{~``Bate'' meant as a comrade, but abbreviated from brother, and actually a lot like it.}, in no particular order. To Bate Jove, you pushed me to get into machine learning, and encouraged me to go for Master's studies abroad; I'm certain I wouldn't have if it wasn't for you, let alone do a Ph.D. To Bate Gjole, if I were half as good of a friend as you were to me, then I've done well. You know that you'll be my best man one day, right? To Bate Kico (Penzija), thank you for reminding us of the importance of standing firm regardless of the circumstances. To Bate Milche, it's selfish of me to only call you whenever something ``hurts'', and I hope to compensate by bringing you andalouse and samurai sauces regularly. To Bate Mrke, I told Dina I was feeling down right after we drove you to the airport, to which, she replied: ``Of course, Mrke is your soulmate.'' I'll leave it at that. To Bate Neno, when I was at my lowest, I bought a one-way ticket to your place in Markdorf. You welcomed me and showed me what genuine hospitality means. I probably would have quit the Ph.D. altogether if it wasn't for you at that time. To Bate Koco, for being someone I have leaned on, from when we were fifteen talking on the bus-stop bench after school, throughout today. To Bate Trkster, you were a constant support to me before you were you and I was me. Hopefully, I was the same to you. To all of you, once again, whatever I write here will \textit{never} do justice to all that you've done for me, and still do. To the other people I know from a long time ago (some are my cousins too), but spend less time with than I should: Dea, Elena and Didi. Thank you for, you know, just being there for me and all the laughs together.

To Beti and Pavle, your support, smoked salmon, and hospitality means the world. Endless thanks for all you did and still do for us, time after time. To Violeta, for being a genuinely good person, and the trileche! To Didi and Marin (my aunt and uncle), for the dinners when I come home, the vacations, and for often feeling like I have a second set of parents.

To Soci and Ljupcho (my mother and father): I could dedicate an entire chapter to listing the countless things you have done and continue to do for me. You walked me to school, supported my basketball games, stood by me when I was an inexperienced 17-year-old trying to freelance, and when I impulsively decided to try my luck abroad, you provided me with the utmost support. I could go on and on, but I’ll leave it at this: If, one day, I can be half as good a parent as you have been to me, I will have done just fine. To my late grandmother, Sultana: I think about you far more than I express, and I know that if you were here today, you would have been the happiest.

To Dina, as Djordje Balasevic says: ``Moj mali verni Sančo Pansa, moja ljubavnica, saborac, i moj najbolji drug\footnote{Đorđe Balašević - Na Bogojavljensku noć}''.
You were my companion through the mood swings, the highs and lows, the daydreaming and night distress, the moments of closeness and the times of farawayness.
Through it all, you remained by my side, which I'm eternally grateful for, and often wonder why.

Lastly, I recall a saying from Trksterot: ``We are merely the average of the people around us.'' I strive to be the average of you all, and therefore, I dedicate this thesis to each and every one of you. You are the pillars of my well-being.

\begin{flushright}
Gorjan Radevski, \\
Antwerp, June 2024
\end{flushright}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/publications/publications.tex <==
\chapter{List of publications}\label{ch:publications}

(*) denotes equal contribution

\textbf{\large{Articles in international peer-reviewed conferences or journals}}

\begin{itemize}
    \item \underline{Radevski, G.}, Collell, G., Moens, M-F., and Tuytelaars, T., (2020). Decoding Language Spatial Relations to 2D Spatial Arrangements. Findings of The Conference on Empirical Methods in Natural Language Processing (EMNLP). \cite{radevski2020decoding}
    \item Grujicic*, D., \underline{Radevski*, G.}, Tuytelaars, T., Blaschko, M., (2020). Learning to ground medical text in a 3D human atlas. The Conference on Computational Natural Language Learning (CoNLL). \cite{grujicic-etal-2020-learning}
     \item \underline{Radevski, G.}, Moens, M-F., and Tuytelaars, T. (2021). Revisiting Spatio-Temporal Layouts for Compositional Action Recognition. The British Machine Vision Conference (BMVC).
     \item \underline{Radevski*, G.}, Grujicic*, D., Blaschko, M., Moens, M-F., Tuytelaars, T., (2023). Multimodal Distillaton for Egocentric Action Recognition. International Conference on Computer Vision (ICCV).
     \item \underline{Radevski, G.}, Gashteovski, K., Hung, C-C., Lawrence, C., Glavaš, G., (2023). Linking Surface Facts to Large-Scale Knowledge Graphs. The Conference on Empirical Methods in Natural Language Processing (EMNLP). \cite{radevski-etal-2023-linking}
     \item Roth*, J. A., \underline{Radevski*, G.}, Marzolini, C., Rauch, A., Günthard, H. F., Kouyos, R. D., Fux, C A., Scherrer, A. U., Calmy, A., Cavassini, M., and others. Cohort-derived machine learning models for individual prediction of chronic kidney disease in people living with Human Immunodeficiency Virus: A prospective multicenter cohort study. The journal of infectious diseases. \cite{roth2021cohort}
     % \item Kalajdziski, S., \underline{Radevski, G.}, Ivanoska, I., Trivodaliev, K., Risteska Stojkoska, B., (2018). Cuisine classification using recipe's ingredients. The International Convention on Information and Communication Technology, Electronics and Microelectronics (MIPRO). \cite{kalajdziski2018cuisine}
\end{itemize}

\textbf{\large{Articles in international peer-reviewed workshops}}

\begin{itemize}
    \item Grujicic*, D., \underline{Radevski*, G.}, Tuytelaars, T., Blaschko, M., (2020). Self-supervised context-aware Covid-19 document exploration through atlas grounding. ACL 2020 Workshop on Natural Language Processing for COVID-19 (NLP-COVID). \cite{grujicic2020self}
     \item \underline{Radevski*, G.}, Grujicic*, D., Blaschko, M., Moens, M-F., Tuytelaars, T., (2022). Students taught by multimodal teachers are superior action recognizers. The 2nd International Ego4D Workshop @ European Conference on Computer Vision (ECCV). \cite{radevski2022students}
\end{itemize}

\textbf{\large{Preprints}}

\begin{itemize}
    \item Popordanoska*, T., \underline{Radevski*, G.}, Tuytelaars, T., Blaschko, M., (2023). Estimating calibration error under label shift without labels. \cite{popordanoska2023estimating}
\end{itemize}

==> mycoverpage.tex <==
% Redefine in this file the commands to generate the front and back cover:
%
%   \makefrontcovergeneral{xskip}{clearpage}
%   \makebackcovergeneral{xskip}{clearpage}
%
% You can start from their definition in adsphd.cls. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My own cover page
\makeatletter

%% \renewcommand{\makefrontcovergeneral}[2]{%
%%   %
%%   % Create header
%%   \frontcoverheader{#1}
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Title, subtitle, authorname, text and date can be moved around.
%%   % Change the textblock* commands below. 
%%   %
%%   % Syntax of textblock environment:
%%   % 
%%   %   \begin{textblock*}{width}(xpos,ypos)
%%   %     ...
%%   %   \end{textblock*}
%%   % 
%%   % !! Make sure not to remove the '+#1' part!!!
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Place the title
%%   \begin{textblock*}{120mm}(17.5mm+#1,89.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \raggedright\selectfont\LARGE\sffamily\textbf{\@title}
%%   \end{textblock*}
%%   %
%%   % Place the subtitle
%%   \begin{textblock*}{120mm}(17.5mm+#1,92.0mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily{\@subtitle}
%%   \end{textblock*}
%%   %
%%   % Place the author name
%%   \begin{textblock*}{120mm}(17.5mm+#1,109.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily\@authorf\ \MakeUppercase\@authorl
%%   \end{textblock*}
%%   %
%%   %\begin{textblock}{120}(0,115)
%%   \begin{textblock*}{120mm}(17.5mm+#1,132.0mm)
%%   \textblockcolour{}
%%   \includegraphics*{image/coverfigure}
%%   \end{textblock*}
%%   %
%%   % Place the misc text
%%   \begin{textblock*}{60mm}(96.5mm+#1,187.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   {\small\sffamily Dissertation presented in partial\\
%%   fulfillment of the requirements for\\
%%   the degree of Doctor\\
%%   in \@degree}
%%   \end{textblock*}
%%   %
%%   % Place date
%%   \begin{textblock*}{160mm}(0mm+#1,221.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \begin{center} {\small\sffamily\@date }\end{center}
%%   \end{textblock*}
%%   
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Add footer
%%   \frontcoverfooter{#2}
%% 
%% }

\makeatother

